Vision Transformer Neural Architecture Search for Out-of-Distribution Generalization: Benchmark and Insights

While ViTs have achieved across machine learning tasks, deploying them in real-world scenarios faces a critical challenge: generalizing under OoD shifts. A crucial research gap exists in understanding how to design ViT architectures, both manually and automatically, for better OoD generalization. To this end, we introduce OoD-ViT-NAS, the first systematic benchmark for ViTs NAS focused on OoD generalization. This benchmark includes 3000 ViT architectures of varying computational budgets evaluated on 8 common OoD datasets. Using this benchmark, we analyze factors contributing to OoD generalization. Our findings reveal key insights. First, ViT architecture designs significantly affect OoD generalization. Second, ID accuracy is often a poor indicator of OoD accuracy, highlighting the risk of optimizing ViT architectures solely for ID performance. Third, we perform the first study of NAS for ViTs OoD robustness, analyzing 9 Training-free NAS methods. We find that existing Training-free NAS methods are largely ineffective in predicting OoD accuracy despite excelling at ID accuracy. Simple proxies like Param or Flop surprisingly outperform complex Training-free NAS methods in predicting OoD accuracy. Finally, we study how ViT architectural attributes impact OoD generalization and discover that increasing embedding dimensions generally enhances performance. Our benchmark shows that ViT architectures exhibit a wide range of OoD accuracy, with up to 11.85% improvement for some OoD shifts. This underscores the importance of studying ViT architecture design for OoD. We believe OoD-ViT-NAS can catalyze further research into how ViT designs influence OoD generalization.

==> appx_sections/additional_figures.tex <==
\section{Main paper figures for other datasets} \label{Sec:Appx_Figures}

\subsection{Example Image of Corruptions in ImageNet-C}\label{sec:Appx_Figures_Imagenetc}

\begin{figure}[H]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.35]{figures/imagenet_c_examples.png}
	% figure caption is below the figure
	\caption{ An example image of IN-C (ImageNet-C) \cite{Hendrycks2018} with different corruption types at different severity levels.  }
	\label{fig:imagenet-c-example}       % Give a unique label
\end{figure}




\subsection{Visualization of OoD Accuracy Range}\label{sec:Appx_Figures_accuracy_range}

\begin{figure}[H]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,width = 14cm]{figures/violin_acc_19.png}
	% figure caption is below the figure
	\caption{Accuracy range over all unique architectures in our OoD-ViT-NAS benchmark. The numbers within each violin plot for each sub-figures (e.g., IN-C Fog 8.89(1.06), 8.00(2.25), and 5.54(0.56)) denote the corresponding OoD(ID) accuracy range of architectures sampled from AutoFormer-Tiny/Small/Base search space, respectively.}\label{fig:benchmark_accuracy_range}       % Give a unique label
\end{figure}
\subsection{ImageNet-C Common Corruption Accuracies}\label{sec:Appx_Figures_inc_accuracy}
Here, we compare the ID/OoD accuracy range of 3000 architectures with varying ViT architectures to capture a different aspect of robustness generalization. \somayeh{include 5 levels of corruption violin plot}

\subsection{ImageNet-P Accuracies}\label{sec:Appx_Figures_inp_accuracy}



\subsection{Effect of ViT Architectural Design on OoD Robustness}\label{Sec:Appx_Figures_Embedding}

\subsubsection{Additional correlation analysis }\label{Sec:Appx_Arch_Correlation}

\somayeh{we will include detailed dataset correlation and proxy correlation for each supernet}
\subsubsection{Effect of embedding dimension on OoD generalization }\label{Sec:Appx_Figures_Embedding}

In our ablation study, we look at the correlation between embedding dimension and ID/OoD accuracy. We fix the network depth at 13 layers while varying the embedding dimension. The result is shown in Figure \ref{fig:ablation-edim}. We find an overall positive correlation of 0.627, suggesting that the embedding dimension can be a good indicator of the model's robustness. For example, higher embedding dimensions improve performance in synthetic corruption of IN-C but are less effective for synthetic images generated in the IN-D dataset, where the correlation becomes close to zero or even negative (as shown in Figure \ref{fig:embedding} and \ref{fig:ablation-edim}). 


\begin{figure}[!ht]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.40]{figures/id_ood_arch_heatmap_small_embed.png}
	% figure caption is below the figure

	\caption{Ablation study on different embedding dimensions on ID/OoD generalization. Kendall rank correlation coefficient between ID/OoD accuracies and embedding dimension for 325 architectures with 13-layer depth. This plot shows a positive correlation between Embed\_Dim and ID/OoD accuracies for most OOD shift datasets, whereas, for IN-D, the correlation becomes close to zero or even negative.  }
	\label{fig:ablation-edim}       % Give a unique label
\end{figure} 

\begin{figure}[!htb]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.30]{figures/embedding_dim/id_ood_embedding_small_27.png}
	% figure caption is below the figure
	\caption{As in Figure \ref{fig:embedding}, we show that higher ID/OoD accuracy can be obtained by increasing the embedding dimension of architectures sampled from \textbf{AutoFormer-Small}. Our observation shows that increasing the network depth does not have a high impact on OoD robustness.   }
	\label{fig:embedding-all-small}       % Give a unique label
\end{figure}


%\begin{figure}[htb!]
%	\centering
%	% Use the relevant command to insert your figure file.
%	% For example, with the graphicx package use
%	\includegraphics[keepaspectratio,scale=0.30]{figures/embedding_dim/id_ood_embedding_small_14.png}
%	% figure caption is below the figure
%	\caption{As in Figure \ref{fig:embedding}, we show that higher ID/OoD accuracy can be obtained by increasing the embedding dimension of ViT blocks. Our observation shows that increasing the network depth does not have a high impact on OoD robustness.   }
%	\label{fig:embedding-all}       % Give a unique label
%\end{figure}


\begin{figure}[!htb]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.30]{figures/embedding_dim/id_ood_embedding_base_all.png}
	% figure caption is below the figure
	\caption{The effect of \#Embed\_Dim on robustness generalization of 1000 architectures sampled from \textbf{AutoFormer-Base}.} % we show that higher ID/OoD accuracy can be obtained by increasing the embedding dimension of ViT blocks. Our observation shows that increasing the network depth does not have a high impact on OoD robustness.   }
	\label{fig:embedding-all-base}       % Give a unique label
\end{figure}


\begin{figure}[!htb]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.30]{figures/embedding_dim/id_ood_embedding_tiny_all.png}
	% figure caption is below the figure
	\caption{The effect of \#Embed\_Dim on robustness generalization of 1000 architectures sampled from \textbf{AutoFormer-Tiny}. }% we show that higher ID/OoD accuracy can be obtained by increasing the embedding dimension of ViT blocks. Our observation shows that increasing the network depth does not have a high impact on OoD robustness.   }
	\label{fig:embedding-all-tiny}       % Give a unique label
\end{figure}

\subsubsection{Effect of Depth}\label{Sec:Appx_Figures_Depth}

Based on Figure \ref{fig:embedding}, for a given embedding dimension (represented by a distinct color), we report the mean accuracy, showing how the mean OoD accuracy changes among ViT architectures of varying depths. We observe that \textit{increasing the network depth does not significantly improve OOD generalization of the architectures in our benchmark}, which aligns with the observations in \cite{Levine2020}. In particular, we observe that ID accuracy with an average-accuracy range of 1.22\% does not change much across all architectures with various numbers of layers (Figure \ref{fig:embedding}, left panel). There, as shown in Figure \ref{fig:embedding-all-small} in Appendix \ref{Sec:Appx_Figures_Embedding}, the average-accuracy range (1.99\%) on our robustness benchmarks is boosted by less than 0.77\%, while the span of mean OoD accuracies remains large, ranging from 0.44\% to 5.86\%. Meanwhile, our analysis also confirms that increasing the depth is not very effective in improving the OoD performance for models sampled from Tiny and Base supernets as well, where the mean OoD accuracies of these networks range in $[0.01,0.92]$ and $[0.05,1.05]$, respectively (see Figure \ref{fig:embedding-all-tiny} and \ref{fig:embedding-all-base}). This indicates that deeper models might not always be beneficial, especially when handling certain OoD distribution shifts. 
% TODO

Figure \ref{fig:depth} depicts the ranking correlation for all architectures between depth and ID/OoD accuracies. In our ablation study, we analyze how variations in the depth parameter affect the model’s robustness by maintaining those architectures with a certain embedding dimension (e.g., Embed\_Dim $=384$). Our analysis shows that increasing the depth can be relatively correlated with high ID accuracy in subnets derived from AutoFormer-Small; however, this increase in depth might not necessarily translate into the OoD distribution shifts and model robustness. This plot shows a positive correlation between the depth for IN-P, IN-R, and IN-A OoD shift, whereas, for all other distribution shifts, the correlation becomes close to zero or even negative. Overall, our findings suggest that increasing network depth significantly narrows the gap between ID and OoD accuracies, indicating that network depth contributes little to OoD robustness in our benchmarks. Further details can be found in Appendix \ref{Sec:Appx_Arch_Correlation}.


%The average OoD classification accuracy results in each depth in Figure \ref{fig:embedding-all-small} (Appendix \ref{appendixB}) also confirm the insignificant effectiveness of depth. Moreover, increasing the network depth 



\begin{figure}[!htb]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.40]{figures/id_ood_arch_heatmap_small_depth.png}
	% figure caption is below the figure
	\caption{Kendall rank correlation coefficient between the network depth and all OoD robust accuracies evaluated on 308 architectures with Embed\_Dim $=384$ and varying depths. The correlation of ranking at bottom is the continuation of rank table of other OoD shifts at the top. }
	\label{fig:depth}       % Give a unique label
\end{figure}

\subsubsection{Effect of MLP Ratio on OoD Generalization }\label{Sec:Appx_Figures_Mlp}



The MLP ratio (or expansion ratio) expands the input embedding dimension by a factor at each layer. To investigate how varying the MLP ratio at each layer affects OoD robustness, we design the layer-wise analysis to investigate the influence of the MLP ratio in each layer by changing the MLP ratio in each layer for our ablation study. 

In AutoFormer-Small search space, the MLP ratio at any given layer — referred to as the $i$-th layer — can be set to 3, 3.5, or 4. We construct a dataset consisting of robust accuracies of 108 randomly sampled from AutoFormer-Small, where the sampled models are fixed with three architectural design components: (Depth = 12, Embed\_Dim = 320, \#Heads = 5). With these parameters fixed, the total number of potential MLP ratio configurations is extensive (i.e., $3^{12}$), making it impractical to evaluate every possible configuration for analysis. Therefore, to specifically assess the influence of the MLP ratio at the $i$-th layer, we maintained a constant MLP ratio across all other layers and then measured the OoD robust accuracies.  Figure \ref{fig:mlp-configuration} in Appendix \ref{Sec:Appx_Figures_Mlp} shows the possible nine configurations of MLP ratio at $5$-th layer. In Table \ref{tab:ablation-mlp}, we observe that changing the MLP ratio at layers \#4 and \#5 leads to an increased range of mean OoD robust accuracy. %Further details can be found in Appendix \ref{Sec:Appx_Figures_Mlp}. 


\input{tables/ablation-mlp.tex} 

\begin{figure}[!htb]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.5]{figures/mlp_layer_configuration.png}
	% figure caption is below the figure
	\caption{The possible configurations of MLP ratio at $5$-th layer of 108 architectures sampled from \textit{AutoFormer-Small} in ablation study. }% we show that higher ID/OoD accuracy can be obtained by increasing the embedding dimension of ViT blocks. Our observation shows that increasing the network depth does not have a high impact on OoD robustness.   }
\label{fig:mlp-configuration}       % Give a unique label
\end{figure}


\begin{figure}[!htb]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.35]{figures/mlp/OOD Acc IN-C Fog 5_all_layers_3.0.png}
	% figure caption is below the figure
	\caption{	A visualization on the effect of changing MLP Ratio per layer to OoD Accuracy in 108 architectures sampled from \textit{AutoFormer-Small} in ablation study. To evaluate the effect of layer $i$-th, we fix the MLP ratio $=3.0$ for the remaining layers. We observe that higher OoD accuracy range can be obtained by changing the MLP ratio at layer 4 and 5. 
	}% we show that higher ID/OoD accuracy can be obtained by increasing the embedding dimension of ViT blocks. Our observation shows that increasing the network depth does not have a high impact on OoD robustness.   }
\label{fig:mlp-configuration1}       % Give a unique label
\end{figure}


\begin{figure}[!htb]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.35]{figures/mlp/OOD Acc IN-C Fog 5_all_layers_3.5.png}
	% figure caption is below the figure
	\caption{A visualization on the effect of changing MLP Ratio per layer to OoD Accuracy in 108 architectures sampled from \textit{AutoFormer-Small} in ablation study. To evaluate the effect of layer $i$-th, we fix the MLP ratio $=3.5$ for the remaining layers.  We observe that higher OoD accuracy range can be obtained by changing the MLP ratio at layer 4 and 5. }% we show that higher ID/OoD accuracy can be obtained by increasing the embedding dimension of ViT blocks. Our observation shows that increasing the network depth does not have a high impact on OoD robustness.   }
\label{fig:mlp-configuration2}       % Give a unique label
\end{figure}

\begin{figure}[!htb]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.35]{figures/mlp/OOD Acc IN-C Fog 5_all_layers_4.0.png}
	% figure caption is below the figure
	\caption{A visualization on the effect of changing MLP Ratio per layer to OoD Accuracy in 108 architectures sampled from \textit{AutoFormer-Small} in ablation study. To evaluate the effect of layer $i$-th, we fix the MLP ratio $=4.0$ for the remaining layers. We observe that a higher OoD accuracy range can be obtained by changing the MLP ratio at layers 4 and 5. }% we show that higher ID/OoD accuracy can be obtained by increasing the embedding dimension of ViT blocks. Our observation shows that increasing the network depth does not have a high impact on OoD robustness.   }
\label{fig:mlp-configuration3}       % Give a unique label
\end{figure}




==> appx_sections/correlation.tex <==
\section{Correlations Between Image Datasets}\label{appendixA}


\subsection{The full correlation matrix}\label{Sec:Appx_Full_Correlation}
We display the full correlation matrix for 3000 subnets architectures sampled from Small, Base, and Tiny supernets in Figure \ref{fig:cor-matrix-small}, \ref{fig:cor-matrix-base}, and \ref{fig:cor-matrix-tiny}, respectively. It shows the pair-wise Kendall rank correlation coefficient between all combinations of ID and OoD distribution shifts. 


\begin{figure}[H]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.60]{figures/id_imagnetc_heatmap_small.png}
	% figure caption is below the figure
	\caption{Kendall rank correlation coefficient between ID and OoD accuracies computed on all 1000 AutoFormer-S architectures. Measurements are computed on different OoD tasks including algorithmically generated corruptions in IN-C and natural distribution shifts in IN-A, IN-D, IN-R, IN-P, and IN-Sketch. The matrix shows the predictiveness of ID accuracy of OoD accuracy. The higher positive values indicate a positive link between ID/OoD accuracies. For some corruption tasks, e.g., Motion and Blur corruption tasks, ID accuracy is less predictive of OoD accuracies. }%The trend for IN-D do not correspond to in OOD performance }%This information is shown separately as a one-row plot in Figure \ref{fig:id-ood-cor-heatmap} in the main text.}
	\label{fig:cor-matrix-small}       % Give a unique label
\end{figure}

\begin{figure}[H]
\centering
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
\includegraphics[keepaspectratio,scale=0.60]{figures/id_imagnetc_heatmap_base.png}
% figure caption is below the figure
\caption{Kendall rank correlation coefficient between ID and OoD accuracies computed on all 1000 AutoFormer-B architectures. Measurements are computed on 15 different algorithmically generated corruptions in ImageNet-C. The matrix shows mostly uncorrelated ranking towards different kinds of common corruptions based on architectural design.  }
\label{fig:cor-matrix-base}       % Give a unique label
\end{figure}

\begin{figure}[H]
\centering
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
\includegraphics[keepaspectratio,scale=0.60]{figures/id_imagnetc_heatmap_tiny.png}
% figure caption is below the figure
\caption{Kendall rank correlation coefficient between ID and OoD accuracies computed on all 1000 AutoFormer-T architectures. The mostly uncorrelated ranking and negative values indicate that ID accuracy is less predictive of OoD accuracies based on architectural design.}
\label{fig:cor-matrix-tiny}       % Give a unique label
\end{figure}


\subsection{Analyzing shift-type correlation}\label{Sec:Appx_Shift_correlation}

For a detailed overview of how good ID accuracy is predictive of OoD accuracy, we investigate the OoD-specific correlation analysis on some severe cases of distribution shift. To this end, we follow the same procedure as described \cite{Wenzel2022} to observe the typical ID/OoD correlation patterns using scatter plots of ID/OOD accuracy. First, we average the OoD accuracies (for all tasks) of all architectures sampled from the AutoFormer-S supernet and compute the ranking correlation of the corresponding (ID and OoD) accuracy pairs. For instance, inspecting Figure \ref{fig:id-ood-cor}, the correlation between ID and the averaged OoD accuracies of corrupted ID is 0.65. By looking at this number, the increasing correlation line reflects that ID classification accuracy positively correlates with the OoD corrupted accuracies in AutoFormer-S architectures. However, our extended set of experiments on 2000 architectures sampled from AutoFormer-B and AutoFormer-T shows that the presence of OoD-specific and architecture-specific factors cannot always show a clear linear trend between ID and OoD classification performance (i.e., accuracy). For (ID, OoD) dataset pairs in AutoFormer-B architectures, we observe a variety of ID and OoD accuracies across 1000 architectures, where ID and OoD accuracies are hardly correlated (Figure \ref{fig:correlation-pattern-base}). Our observation shows that OoD generalization can change on different OoD distribution shifts. For example, the horizontal line correlation trend between ID and OoD accuracies evaluated on architectures sampled from AutoFormer-T indicates that a variety of subnets sampled within limited $5\text{M} \thicksim7\text{M}$ parameter range do not necessarily behave very differently from one another (Figure \ref{fig:correlation-pattern-tiny}, right panel) in terms of robustness and OoD generalization. Furthermore, we display the correlation matrix between ID and OoD common corruptions of ImageNet-1K in Figure \ref{fig:id-ood-cor-heatmap}. %Hence, ID accuracy is not a good criterion for obtaining robust % The full pair-wise correlation coefficient matrix is computed as described in Appendix \ref{appendixA}. 


%where the accuracy improvement on ID test data translates to a larger accuracy improvement on the OoD data \cite{Recht2019}.
% While evaluations of various aspects of ViTs has been done \cite{bibid}, its robustness, i.e., the performance of model on the new held-out test dataset, is still unclear. 

\begin{figure}[htb]
	\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[keepaspectratio,scale=0.45]{figures/id_ood_accuracy_correlation.png}
	% figure caption is below the figure
	\caption{Scatter plot patterns in our dataset. Kendall rank correlation coefficient is computed for 1000 subnet architectures sampled from \textit{AutoFormet-S} supernet. \textit{Increasing line:} ID and averaged ImageNet-C OoD accuracies nearly lie ``on a line".}
	\label{fig:id-ood-cor}       % Give a unique label
\end{figure}


\begin{figure}[H]
	\centering
	\begin{subfigure}[b]{0.49\textwidth} % Adjust width to fit your needs
		\includegraphics[width=0.9\textwidth]{figures/id_ood_accuracy_correlation_base.png}
		%\caption{Image 1}
		%\label{fig:autoformer-b}
	\end{subfigure}
	%\hfill % This command adds space between the subfigures
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.9\textwidth]{figures/id_contrast_accuracy_correlation_base.png}
		%\caption{OoD-specific }
		%\label{fig:autoformer-s}
	\end{subfigure}
	
	\caption{Scatter plot patterns in our datasets for 1000 architectures in \textit{AutoFormer-B}. ID and averaged ImageNet-C OoD accuracies are mostly uncorrelated. \textit{No clear trend:} architectures sampled from \textit{AutoFormer-B} show a variety of ID and OOD accuracies. This means similar ID accuracies are obtained while they differ in their performance for OoD generalization.    }
	\label{fig:correlation-pattern-base}
\end{figure}



\begin{figure}[htb]
	\centering
	\begin{subfigure}[b]{0.49\textwidth} % Adjust width to fit your needs
		\includegraphics[width=0.9\textwidth]{figures/id_ood_accuracy_correlation_tiny.png}
		%\caption{Image 1}
		
	\end{subfigure}
	%\hfill % This command adds space between the subfigures
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=0.9\textwidth]{figures/id_contrast_accuracy_correlation_tiny.png}
		%\caption{OoD-specific }
		
	\end{subfigure}
	
	\caption{Scatter plot patterns in our datasets for 1000 architectures in \textit{AutoFormer-T}. ID and averaged IN-C OoD accuracies are hardly correlated. \textit{Horizontal line, low OoD accuracy:} models have very poor OoD performance despite having a variety of different ID accuracy. The presence of severe OoD shift is observed in IN-C Contrast OoD distribution shift (i.e., OoD-specific factor).  }
	\label{fig:correlation-pattern-tiny}
\end{figure}





==> appx_sections/related_work.tex <==
\section{Related Work} \label{Sec:Appx_Related_work}

\textbf{Vision Transformers (ViTs).} ViTs are a rapidly evolving deep learning architecture in computer vision domain. Unlike Convolutional Neural Networks (CNNs), ViTs leverage attention mechanisms, originally developed for natural language processing \cite{vaswani2017attention}, to capture long-range dependencies within images. This architecture relies on two key components: Channel-wise MLP blocks and Attention blocks. Recently, ViT architectures \cite{dosovitskiy2020image,tu2022maxvit,liu2021swin,chen2021autoformer,wang2023prenas,li2022exploring,zhang2022segvit} demonstrate impressive performance across various computer vision tasks.

\textbf{Out-of-Distribution (OoD) Generalization}. Addressing Out-of-distribution (OoD) generalization in machine learning is challenge, particularly in computer vision. Various approaches have been proposed to tackle OoD domain shifts robustness. A common strategy focuses on learning features that remain consistent across different domains, promoting generalizability  \cite{arjovsky2019invariant,ghifary2015domain,mahajan2021domain,muandet2013domain,rame2022fishr,rojas2018invariant,shi2021gradient}. Other research directions explore distributional robustness \cite{sagawa2019distributionally,zhou2020learning}, model ensembles \cite{chen2023explore,rame2023model}, test-time adaptation \cite{park2023test,chen2023improved}, data augmentation techniques \cite{nam2021reducing,chen2022self,kim2021selfreg,li2021simple,zhou2021domain,xu2021fourier,yan2020improve}, and meta learning \cite{du2020metanorm,shu2021open} for improved OoD performance. From architectural perspective, a few attempts investigates the impact of network architecture on OoD generalization. Early work \cite{sagawa2020investigation} shows that that over-parameterized networks can hinder OoD performance due to overfitting. This raises an intriguing question: can sub-networks within such architectures achieve better OoD results? Inspired by the Lottery Ticket Hypothesis \cite{frankle2018lottery}, researchers have explored the Functional Lottery Ticket Hypothesis proposing that over-parameterized networks harbor sub-networks with superior OoD capabilities. Techniques like Modular Risk Minimization (MRM) \cite{zhang2021can} and Debiased Contrastive Weight Pruning (DCWP) \cite{park2023training} aim to identify these winning tickets. An other direction \cite{bai2021ood,tang2021robustart} leverages Neural Architecture Search (NAS) to analyze the OoD robust architectures. However, these studies primarily focuses on Convolutional Neural Network (CNN) architectures. While ViTs have achieved success in various visual recognition, investigations into their OoD robustness are limited. Initial works \cite{tang2021robustart} and \cite{rahman2023out} evaluate sets of 10 and 22 human-designed ViT architectures under OoD settings, respectively. Their experimental results provide coarse insights into which models exhibit better OoD performance. \textit{However, the influence of  components design on OoD robustness remains unclear.}

\textbf{Neural Architecture Search (NAS)}. NAS is a promising approach and achieves remarkable success in automatically search for efficient and effective architectures for ID performance \cite{wang2021alphanet,yu2020bignas,wang2021attentivenas,jiang2024meco}. Recently, NAS has been explored in the context of adversarial robustness for CNNs as well \cite{jung2023neural,ha2024generalizable,wurobust}. With the rise of Vision Transformers (ViTs), several NAS approaches have been applied to improve ViT architectures, including Autoformer \cite{chen2021autoformer}, S3 \cite{chen2021searching}, ViTAS 
\cite{su2022vitas}, ElasticViT \cite{tang2023elasticvit}, DSS \cite{zhou2022training}, Auto-Prox \cite{wei2024auto} and GLiT \cite{chen2021glit}. Additionally, hybrid CNN-ViT architectures like HR-NAS \cite{ding2021hr}, UniNet \cite{liu2022uninet}, and NASViT \cite{gong2022nasvit} have also been explored. These efforts have shown promising results in terms of ID accuracy. \textit{However, there has not been any work on applying NAS to ViT architectures specifically for OoD generalization.}

==> sections/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}%, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Sec.~\ref{Sec:Benchmark} for our OoD-ViT-NAS benchmark, and Sec.~\ref{Sec:Investigation} for our analysis. The summary can be found in Fig.~\ref{fig:OoDshifts_Visualization}, Fig.~\ref{fig:analysis-investigation}, and Tab.~\ref{tab:benchmark_summary}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}, % \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appx.~\ref{Sec:Limitation}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appx.~\ref{Sec:Appx_Reproducibility}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appx.~\ref{Sec:Appx_Overview} 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appx.~\ref{Sec:Appx_Reproducibility}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Tab.~\ref{tab:proxy}. Our benchmark and analysis are conducted across datasets and search space. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appx.~\ref{Sec:Appx_Reproducibility}, $\sim$ 3900 GPU hours on a single Nvidia RTX A6000
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appx.~\ref{Sec:Limitation}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appx.~\ref{Sec:Appx_Benchmark} and Appx.~\ref{Sec:Appx_Reproducibility} for description of dataset and experimental setups, respectively. We do not mention the license of the assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appx.~\ref{Sec:Appx_Overview} for our OoD-ViT-NAS benchmark. See Sec.~\ref{Sec:Benchmark}, and Appx.~\ref{Sec:Appx_Benchmark} for the description of the benchmark.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

